DocChecker: Bootstrapping Code Large Language Model for Detecting and Resolving Code-Comment Inconsistencies

Comments within source code are essential for developers to comprehend the code's purpose and ensure its correct usage. However, as codebases evolve, maintaining an accurate alignment between the comments and the code becomes increasingly challenging. Recognizing the growing interest in automated solutions for detecting and correcting differences between code and its accompanying comments, current methods rely primarily on heuristic rules. In contrast, this paper presents DocChecker, a tool powered by deep learning. DocChecker is adept at identifying inconsistencies between code and comments, and it can also generate synthetic comments. This capability enables the tool to detect and correct instances where comments do not accurately reflect their corresponding code segments. We demonstrate the effectiveness of DocChecker using the Just-In-Time and CodeXGlue datasets in different settings. Particularly, DocChecker achieves a new State-of-the-art result of 72.3% accuracy on the Inconsistency Code-Comment Detection (ICCD) task and 33.64 BLEU-4 on the code summarization task against other Large Language Models (LLMs), even surpassing GPT 3.5 and CodeLlama. DocChecker is accessible for use and evaluation. It can be found on our GitHub https://github.com/FSoft-AI4Code/DocChecker and as an Online Tool http://4.193.50.237:5000/. For a more comprehensive understanding of its functionality, a demonstration video is available on YouTube https://youtu.be/FqnPmd531xw.

==> source/limitation.tex <==
In practice scenarios, one reason for the misalignment between code and comments is developers making modifications to their code without subsequently updating the comments. Although we introduce a framework for detecting and updating inconsistencies, we do not consider a setting, where both the previous and updated versions of the code and comment are available. In our future work, we intend to delve further into analyzing the changes in the code function before and after updates, while also leveraging the previous version of the comment to generate a new one that aligns with the new version of code snippets.

==> source/task.tex <==
\label{method:finetune}

Developers frequently refactor source code and incorporate new functionality. However, code comments are frequently ignored when changes are made \cite{ratol2017detecting,panthaplackel2021deep,wen2019large},  resulting in a lack of consistency between the code and the comments. Our task is given a comment \textit{$C$} with a corresponding code method \textit{ $M$}, and we have to determine whether the comment \textit{$C$} is semantically out of sync with the code function \textit{$M$}. Following \cite{panthaplackel2021deep}, we address this challenge in two separate settings:
\begin{itemize}
  \item Post hoc setting: In this setting, the code changes that resulted in the mismatch are unknown; Only the current version of the code-comment pair is available.
  \item Just In Time setting: Here, we take into account changes to the code function before and after they are committed to the repository by the developers. Analyzing these modifications may determine which ones lead to inconsistent comments. Therefore, both versions of code function \textit{$M_{old}$} and \textit{$M$} are available with the comment \textit{$C$}.
\end{itemize}
